Understanding Compressive Adversarial Privacy

Designing a data sharing mechanism without sacrificing too much privacy can be considered as a game between data holders and malicious attackers. This paper describes a compressive adversarial privacy framework that captures the trade-off between the data privacy and utility. We characterize the optimal data releasing mechanism through convex optimization when assuming that both the data holder and attacker can only modify the data using linear transformations. We then build a more realistic data releasing mechanism that can rely on a nonlinear compression model while the attacker uses a neural network. We demonstrate in a series of empirical applications that this framework, consisting of compressive adversarial privacy, can preserve sensitive information.

==> discarded/priv_linear_categorical_response.tex <==
\subsection{Linear Compression with Categorical Label} 
Here we consider a scenario that the private labels are discrete, and more specifically, say a sample $i$ that $y_i \in \mathcal{Y}=\{-1, +1\}, x_i \in R^p$. And $x_i^T$ is the $i$-th row of data matrix $X$. Data holder will design a linear compression mechanism to reduce the classification accuracy of $y_i$ given $\tilde{x}_i$, where $\tilde{x}_i=g(x_i, y_i)$, where $g$ is a function applies linear compression. For the attacker here we assume the loss function is logistic loss $\ell_{\theta}(h(\tilde{x}), y) = \sum_{i=1}^N \log(1+\exp(-y_i\theta^T\tilde{x_i})) $. 
The compression operation is performed such that $\tilde{x}_i = AA^{\dagger}{x}_i$ where $A \in R^{p\times k}$ and $A^{\dagger} \in R^{k\times p}$ given the result in equation \ref{linear:sudo:inverseA}. 
%
\begin{align}
& \max_{A}\bigg\{ \min_{\theta}\Big( \sum_{i=1}^N \log(1+\exp(-y_i\theta^T AA^{\dagger}x_i))\Big) \bigg\} \\
& s.t. \quad \|XAA^{\dagger} - X\|_F^2 \leq \gamma
\end{align}
% 
Notice the $AA^{\dagger} = A(A^TA)^{-1}A^T$ is positive semidefinite (see appendix \ref{pes:priv:app:linear:tran:M:psd}). Therefore we solve a relaxed Semidefinite Programming with a rank constraint instead of explicitly solve $A$ for outer maximization. Re-parameterizing $M=AA^{\dagger}$ and applying the nuclear norm regularization to relax the rank constraint given $M$ is PSD, we have 
% \begin{align}
% \max_{M}\bigg\{ \min_{\theta}\Big( \sum_{i=1}^N \log(1+\exp(-y_i\theta^T Mx_i))\Big) \\
% - \gamma\|XM - X\|_F^2\bigg\} \\
% s.t. \qquad rank(M) = k \\
% \qquad\qquad M \succeq 0
% \end{align} 
\begin{align}
& \max_{M}\bigg\{ \min_{\theta}\Big( \sum_{i=1}^N \log(1+\exp(-y_i\theta^T Mx_i))\Big) - \beta \|M\|_{*} \bigg\} \\
& s.t.  \quad \|XM - X\|_F^2 \leq \gamma  \\
& \qquad M \succeq 0 
\end{align}
we solve this game by using stochastic gradient decent method between attacker and data holder interactively, terminate the procedure when $\theta$ converges and $M$ satisfies the rank $k$. Given a $M$, the attacker's loss gradient is $
\nabla_{\theta}\ell = -\sum_{i=1}^N \sigma(-y_i\theta^T\tilde{x}_i)y_i \tilde{x}_i =-\sum_{i=1}^N \sigma(-y_i\theta^T M {x}_i)y_iM{x}_i $
where $\sigma(z)=1/(1+\exp(-z))$ is the sigmoid function. 
The Hessian of logistic loss is $H_{\theta} = \sum_{i=1}^N\sigma(\theta^T\tilde{x}_i)\sigma(-\theta^T\tilde{x}_i)\tilde{x}_i\tilde{x}_i^T = \sum_{i=1}^N\sigma(\theta^TM{x}_i)\sigma(-\theta^TM{x}_i)M{x}_i {x}_i^TM^T$. Since $M$ is positive semidefinite, it's easy to discover that the Hessian $H_{\theta}$ is also positive semidefinite. Thus the inner minimization problem is a convex optimization. It has been discovered that a few samples can influence the attackers model parameter $\theta$ significantly, and with a linear transformation $M$ these effects could be amplified. We solve the $M$ and $\theta$ iteratively. A simple Algorithm \ref{pes:priv:alg:linear:gen:X_tilde:categ} is given as follows 
%
\begin{algorithm}[ht]
\caption{Generating $\tilde{X}$ w/ categorical label (Linear attacker)}
\label{pes:priv:alg:linear:gen:X_tilde:categ}
\begin{algorithmic}[1]
\STATE \textit{Input:} dataset $(X, Y) \in \mathcal{D}$, iteration $T$, desired rank $k$ \\
\STATE \textit{Output:} $M, \tilde{X}$ \\
\STATE partition dataset into several batches ($X, Y$) \\
\FOR {a batch of ($X, Y$)} 
	\STATE initialize $t=0$, $M_t = I$, $\gamma_t, \beta_t$ for some value \\
    \STATE $\theta_t = \arg \min_{\theta}\frac{1}{N} \sum_{i=1}^N \log(1+\exp(-y_i\theta^T M_t x_i))$
    \WHILE {$t < T$}
    \STATE $t=t+1$\\
        \STATE $M_{t} = \big\{ \arg\max_{M} \frac{1}{N} \sum_{i=1}^N \log(1+\exp(-y_i\theta_t^T Mx_i))-\beta_t \|M\|_{*}$  \\
        s.t. $\sum_{i=1}^N \sigma(-y_i\theta_t^T M {x}_i)y_iM{x}_i = 0 $;\\
            $\quad \|XM - X\|_F^2 \leq \gamma \big\}$
        \STATE $\theta_t \gets \arg \min_{\theta}\frac{1}{N} \sum_{i=1}^N \log(1+\exp(-y_i\theta^T M_{t} x_i))$
        \STATE $U_t, \Lambda_t \gets $ SVD($M_t$) where $M_t = U_t\Lambda_tU_t^T$ 
        \STATE $ \hat{k} = \tilde{rank}(\Lambda_t)$. check the rank of the matrix $\Lambda$ with non trivial eigenvalues. (e.g $\lambda_j > \eta \lambda_{max}, \text{where } \forall j =1,\hdots,n; \eta = 0.01$.) 
  \IF {$\hat{k} = k $ and $\|M_t - {M_{t-1} }\|_F \leq \epsilon$ } 
  \STATE break
  \ELSIF {$\hat{k} > k $}
  \STATE $\beta_{t+1} \gets \beta_t + \frac{\beta_t}{2}$
  \ELSIF {$\hat{k} < k $} 
  \STATE $\beta_{t+1} \gets \beta_t - \frac{\beta_t}{4} $ 
  \ENDIF 
        
    \ENDWHILE
   \STATE $M = \frac{1}{T}\sum_{t=1}^T M_t$; $\tilde{X} = XM$
\ENDFOR
\end{algorithmic}
\end{algorithm}


